Optimal Kernel Orchestration for Tensor Programs with Korch

Kernel orchestration is the task of mapping the computation defined in different operators of a deep neural network (DNN) to the execution of GPU kernels on modern hardware platforms. Prior approaches optimize kernel orchestration by greedily applying operator fusion, which fuses the computation of multiple operators into a single kernel, and miss a variety of optimization opportunities in kernel orchestration. This paper presents Korch, a tensor program optimizer that discovers optimal kernel orchestration strategies for tensor programs. Instead of directly fusing operators, Korch first applies operator fission to decompose tensor operators into a small set of basic tensor algebra primitives. This decomposition enables a diversity of fine-grained, inter-operator optimizations. Next, Korch optimizes kernel orchestration by formalizing it as a constrained optimization problem, leveraging an off-the-shelf binary linear programming solver to discover an optimal orchestration strategy, and generating an executable that can be directly deployed on modern GPU platforms. Evaluation on a variety of DNNs shows that Korch outperforms existing tensor program optimizers by up to 1.7x on V100 GPUs and up to 1.6x on A100 GPUs. Korch is publicly available at https://github.com/humuyan/Korch.

==> rules.tex <==
\section*{========== Old versions =========}













































\section{Derivation Rules}
\label{sec:rules}

\begin{table*}[h]
\centering
\caption{Derivation rules for tensor algebra expressions}
\label{tab:derivation-rules}
\vspace{-0.5em}
\begin{tabular}{cll}
\toprule
& Rules & Descriptions \\ \midrule
\multirow{5}{*}{\shortstack[m]{Intra-expression \\ derivation}} 
& Summation splitting & Split summation from one \stages into two  \\ %
& Variable substitution & Replace iterators of traversal operations with new ones \\ %
& Traversal merging & Merge two \stages into one by merging traversals  \\ %
& Boundary relaxing & Relax the range of iterators \\ 
& Boundary tightening  & Tighten  the range of iterators \\ 
\midrule

\multirow{3}{*}{\shortstack[m]{Inter-expression \\ derivation}}  & Expression splitting & Split an expression into multiple independent expressions \\ 
& Expression merging & Merge multiple independent expressions into one \\ 
& Expression fusion & Fusing multiple dependent expressions into one \\ 
\midrule

\multirow{2}{*}{\shortstack[m]{Expression \\ instantiation}} 
& Operator matching & Match a \stage with operators and replace it by a tensor \\
& \eop generation & Generate an \eop for a scope and replace it by a tensor \\ 
\bottomrule
\end{tabular}%
\end{table*}

\begin{figure*}[h!]
    \centering
    \includegraphics[width=0.95\linewidth,keepaspectratio]{figures/conv2gemm-expr.pdf}
    \vspace{-1em}
    \caption{The derivation process of the example in \Cref{fig:conv2gemm}, which replaces {\tt Conv} with {\tt Matmul} and \eops}
    \label{fig:conv2gemm-expr}
    \vspace{-.5em}
\end{figure*}



Tensor algebra expressions have numerous transformations involving both computation and data layout. 
But there is a lack of formal definition for them.
In \Cref{tab:derivation-rules}, we summarize three classes of rules for expression  transformations, including intra-expression transformation, inter-expression transformation, and expression instantiation. \sys further designs directional derivation based on them to efficiently discover optimizations. 
This design 
maintains the correctness during derivation by the math equivalence behind derivation rules, covers numerous existing tensor program optimizations, and discovers new ones. 






\para{Intra-expression derivation} transforms expressions according to the view of computation, including reorganizing computing workload and rewriting the expressions for fixed computing workload.
\sys uses intra-expression derivation rules to derive expressions to have a similar computation patterns with target operators.

\para{Inter-expression transformation} enables \sys{} to perform optimizations across different expressions. 

\para{Expression instantiation} lowers expressions into executable kernels.
\sys instantiates an invocation of well-optimized library kernels or code-generated kernels for them.
After applying these rules, the instantiated scope is replaced with a tensor in the original expression and separated from the following derivation. 







\Cref{fig:conv2gemm-expr} shows the derivation process of the example in \Cref{fig:conv2gemm}, which transforms a $3 \times 3$ convolution to $9$ \texttt{Matmul} and an \texttt{OffsetAdd} \eop. 
In the following subsections, we will using this example to explain how the rules in \Cref{tab:derivation-rules} work.

\subsection{Intra-Expression Derivation}
\label{sec:compute-rule}


\para{Summation splitting} divides an summation operator into two \stages by applying the following summation rules:
\begin{align*}
 \opL_{\vec{x}}\sum_{\vec{s_1},\vec{s_2}}f(\mathT\pos{\vec{x},\vec{s_1},\vec{s_2}})\Rightarrow\opL_{\vec{x}}\sum_{\vec{s_1}}\{\opL_{\vec{x}\vec{s_1}}\sum_{\vec{s_2}}f(\mathT\pos{\vec{x},\vec{s_1},\vec{s_2}})\}[\vec{x},\vec{s_1}]   
\end{align*}
\cred{where where $\mathbf{\tau}$ is an index computation function.}
\sys divides the iterators of summation operation into two groups, $\vec{s_1}$ and $\vec{s_2}$, and the summation operator is split into two nested \stages $\m{S}_1, \m{S}_2$, i.e., $\m{S}_1=\opLd_{\vec{x}\vec{s_1}}\sumd_{\vec{s_2}}f(\mathT\pos{\vec{x},\vec{s_1},\vec{s_2}})$ and $\Stage_2=\opLd_{\vec{x}}\sumd_{\vec{s_1}}\Stage_1[\vec{x},\vec{s_1}]$.

To transform a 3$\times$3 convolution to a batch of nine matrix multiplications, as shown in \Cref{fig:conv2gemm-expr}, we first transform the initial tensor expression in line (1) to line (2) by separating the iterators $c$ from the other two iterators $r$ and $s$.
The inner \stage only sums along the $c$ dimension; as a result, an intermediate $5$-dimensional tensor is generated since the summation along $r$ and $s$ is not performed but converted to iterators of a traversal operator.
The outer \stage computes the remaining summation over the two extra dimensions created by $r$ and $s$.
Finally, a $4$-dimensional tensor is generated, which is equivalent to the original result. 
The corresponding computation graph is transformed from \Cref{fig:conv2gemm-expr} (a) to (b) after summation splitting.





\para{Variable substitution} substitutes a group of iterators with new ones.
To maintain equivalence and determine the range of the new variables, we perform variable substitution based on the following rules: 

For an iterator space $\mathbb{X}$, 
if there is a {\em bijective} function $\Phi$ that maps elements in $\mathbb{X}$ to another iterator space, then

\begin{align*}
\opL_{\vec{x}}^\mathbb{X}f(\mathT\pos{\vec{x}})\Rightarrow\opL_{\vec{x}}^\mathbb{X}\{\opL_{\vec{y}}^{\Phi(\mathbb{X})}f(\mathT\pos{\Phi^{-1}(\vec{y})})\}[\Phi(\vec{x})]
\end{align*}
, where $\Phi^{-1}$ is the reverse function of $\Phi$, i.e., $\Phi^{-1}(\Phi(\mathbb{X}))=\mathbb{X}$.
This rule implies how to construct an intermediate \stage with new iterators and preserves equivalence.
$\Phi$ maps an iterator space $\mathbb{X}$ to a new one, $\Phi(\mathbb{X})$. $\vec{x}$ and $\vec{y}$ \cred{in \Cref{eq:var-sub} are} the iterators before and after the variable substitution, respectively.
The reverse function $\Phi^{-1}$ is used to construct the new tensor expression. 

In the running example in \Cref{fig:conv2gemm-expr}, \sys applies variable substitutions to transform the tensor algebra expression from line (2) to line (3), using the following injective function: $(r,s,f,t_1,t_2)=\Phi(r,s,h,w,f)=(r,s,f,h+r,w+s)$. Specifically, $h+r$ and $w+s$ are substituted with $t_1$ and $t_2$.
After the variable substitution, the computation graph remains unchanged.



\para{Traversal merging} merges traversal operators in two \stages into a single \stage by applying the \stage derivation rules. 
The following formula shows how traversal merging is performed:
\begin{align*}
\opL_{\vec{x}}^\mathbb{X}\{\opL_{\vec{y}}^\mathbb{Y}f(\mathT\pos{\vec{y})}\}[\Phi(\vec{x})]\Rightarrow\opL_{\vec{x}}^\mathbb{X}f(\mathT\pos{\Phi(\vec{x})})
\end{align*}
, where $\Phi(\mathbb{X}) \subseteq \mathbb{Y}$. 
This rule merges the iterator spaces of two traversal operators into one by applying the mapping function between the two iterator spaces.

For the example in \Cref{fig:conv2gemm-expr}, \sys applies traversal merging to transform the tensor algebra expression from line (4) to line (5) by merging the two outer \stages.
The traversal merging is applied using the mapping function $\Phi(r,s,h,w,f)=(r,s,f,h+r,w+s)$.
After the traversal merging, a \stage is removed, and the computation graph remains unchanged. 





\para{Boundary relaxing and tightening} inspects whether some output can by avoided if they have constant results for any inputs.   
\sys executes constant propagation on tensor algebra expressions to deal with constant numbers in expressions and padding in tensors.
If a region of output has constant value, \sys converts it into an attribute of tensors to reduce meaningless computation. 
The following formula shows how boundary relaxing and tightening are performed:
\begin{align*}
\opL_{\vec{x}}^\mathbb{X}f(\mathT\pos{\vec{x}}) \Longleftrightarrow \opL_{\vec{x}}^{\mathbb{X}'}f(\mathT\pos{\vec{x}})
\end{align*}
, where $\mathbb{X} \subset \mathbb{X}'$, and computation on $\mathbb{X}' - \mathbb{X}$ will not be used as the results of the tensor program. 

In the running example in \Cref{fig:conv2gemm-expr}, the formula in line (4) performs boundary relaxing on $t_1$ and $t_2$, transforming their ranges from $[0, H+r)$ and $[0, W+s)$ to $[-1, H+1)$ and $[-1, W+1)$, respectively, as $r$ and $s$ are in range of $[-1, 1]$. 
After boundary relaxing, the computation graph is transformed from \Cref{fig:conv2gemm-expr} (b) to (c).
The formula in line (6) performs boundary tightening on on $t_1$ and $t_2$, transforming their ranges from $[-1, H+1)$ and $[-1, W+1)$ to $[0, H)$ and $[0, W)$, respectively, as the computation taken on $t_1 = -1$, $t_1 = H+1$, $t_2 = -1$ and $t_2 = W+1$ will not be used for the output tensor.
After boundary tightening, the computation graph is transformed from \Cref{fig:conv2gemm-expr} (c) to (d).




































{
\color{red}

\subsection{Expression Instantiation}
\label{sec:expre-contraction}

Expression instantiation rules lower expressions into executable kernels.
After applying these rules, the instantiated scope is replaced with a tensor in the original expression and separated from the following derivation. 
\sys supports two classes of instantiation, operator matching and \eop generation, to leverage existing highly optimized kernels and flexibly generate other kernels.  
In this subsection, we will introduce how these two instantiation rules work.


\begin{table}[]
\caption{\Itab}
\label{tab:itab}
\vspace{-0.5em}
\centering
\resizebox{0.46\textwidth}{!}{%
\begin{tabular}{ccc|cccc}
\toprule
\multicolumn{3}{c|}{Tensors}          & \multicolumn{4}{c}{Ops} \\
\hline
input      & weight     & output     & \texttt{Add} & \texttt{Matmul}  & \texttt{Conv}  & \texttt{G2BMM} \\
\hline
\checkmark & \checkmark & \checkmark & $mn$  & $b$       &       & $bm$    \\
\checkmark &            & \checkmark &     & $m$       & $nhw$   &       \\
           & \checkmark & \checkmark &     & $n$       & $f$     & $w$     \\
\checkmark & \checkmark &            &     & $k$       & $crs$   & $k$     \\
\bottomrule
\end{tabular}
}
\end{table}

\subsubsection{Pattern Matching}
\label{sec:rule-pattern-matching}

Mapping a tensor algebra expression to an operator is challenging since an operator can be represented in various expressions with potentially different tensor layouts, tensor shapes, and iterators.
For example, the standard tensor algebra expression of a batched matrix multiplication is shown in Equation~(\ref{eq:bmm}). 
\begin{align}
    \opL_{bmn}\sum_{k}A[b,m,k]B[b,k,n]
    \label{eq:bmm}
\end{align}
\begin{align}
    \opL_{bmn}\sum_{k}C[b,0,m,1+k]D[b-1,b,k,n]
    \label{eq:bmm-variant}
\end{align}
However, although Expression~(\ref{eq:bmm-variant}) is significantly different from Expression~(\ref{eq:bmm}), it can also be directly instantiated as a batched matrix multiplication in math libraries\footnote{Math libraries including BLAS allow for specifying the stride of dimensions to work with different input layouts.}. Similar problems exist for other operators. 


To match a tensor algebra expression to operators, 
\sys uses {\em \itab} to summarize linear algebra properties of expressions.
\Itab supports all operators expressible in tensor algebra expression. \Cref{tab:itab} shows typical operators, including an element-wise operator, matrix multiplication, convolution, and G2BMM~\cite{langer2018band} (general to band matrix multiplication). 
The right part of the table list all iterators of an operator, which are categorized into four groups based on whether the iterators appears in the input, weight, and output tensor. 
\Itab also records the coefficient of iterators in the index of each tensors for operator matching.

Taking the batched matrix multiplication (Expression~(\ref{eq:bmm})) as an example, the iterators $b$, $m$, $n$, and $k$ appear in different combinations of the input, weight, and output tensors.
These variables are assigned to different \emph{iterator groups}, as shown in \Cref{tab:itab}.
To match an expression with a specific operator, we need to match the iterators in this expression to the iterators in the \itab.

The detailed matching process is listed as follows:

\begin{enumerate}[leftmargin=*]
    \item  \textbf{Fill iterators into \itab}: enumerate all the iterators in a given expression, and fill them in into the iterator groups in the \itab according to which tensor it appears in. 
    
    \item \textbf{Match iterator groups}: for each iterator group in \itab, the number of iterators should be the same.
    
    \item \textbf{Match iterators}: if there are multiple iterators in an iterator group, enumerate all one-to-one mapping between variables of the operator and those of the expression. 
    After the variables are mapped, check whether the coefficients of iterators in index match (whether the coefficient of each variable and the correlation between different variables in the expression are consistent with patterns, e.g., $h$ and $r$ should have the same coefficient in the index of input tensor of convolution in Expression~(\ref{eq:conv})). 
    
\end{enumerate}

For the example in Equation~(\ref{eq:bmm-variant}), it has the same iterator groups with \texttt{Matmul}. There is an unique one-to-one iterator mapping between the expression and \texttt{Matmul} and it matches all iterators.
After the pattern match rule succeeds, \sys replaces the matched scope with a tensor and generates a corresponding \texttt{Matmul} operator in the computation graph.

\subsubsection{\eop Generation}
\label{sec:rule-eop-matching}

For expressions which cannot match existing operators, \sys converts them into \eops and generates executable kernels based on their tensor algebra expressions.
Since tensor algebra expressions exactly define the computation semantics, 
\sys is able to feed them into existing code generation frameworks, such as TVM, Halide, and Tiramisu~\cite{baghdadi2019tiramisu}.
For example, for the expression in line (7) of \Cref{fig:conv2gemm-expr}, \sys lowers it to TVM by converting its iterator space of traversal operation into a tensor and the computation expression into a lambda function.
\Cref{fig:codegen} shows the result which can be processed by TVM to automatically generate kernel.
\lz{Only membound/few-computation kernel}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth,keepaspectratio]{figures/codegen-tvm.pdf}
    \caption{Lowering the expression (7) in \Cref{fig:conv2gemm-expr} to TVM.}
    \label{fig:codegen}
\end{figure}

}

\subsection{Inter-Expression Derivation}
\label{sec:inter-expr-rule}

\para{Expression splitting} splits an expression into multiple independent expressions using the following rule:
\begin{align*}
\opL_{\vec{x}}^{\mathbb{X}}f(\mathT\pos{\vec{x}}) \Longrightarrow 
\opL_{\vec{x}}^{\mathbb{X}_1}f(\mathT\pos{\vec{x}}) \sim \opL_{\vec{x}}^{\mathbb{X}_2}f(\mathT\pos{\vec{x}}) 
\end{align*}
where $\mathbb{X} \subseteq \mathbb{X}_1 \cup \mathbb{X}_2$, and $\sim$ denotes that the two expressions have no dependency.

\para{Expression merging} merges multiple independent expressions with the same computation $f(\mathT\pos{\vec{x}})$, which is the symmetric transformation of expression splitting:
\begin{align*}
\opL_{\vec{x}}^{\mathbb{X}_1}f(\mathT\pos{\vec{x}}) \sim \opL_{\vec{x}}^{\mathbb{X}_2}f(\mathT\pos{\vec{x}}) \Longrightarrow \opL_{\vec{x}}^{\mathbb{X}}f(\mathT\pos{\vec{x}})
\end{align*}
where $\mathbb{X}_1 \cup \mathbb{X}_2 \subseteq \mathbb{X}$.

\begin{figure}[]
    \centering
    \includegraphics[width=\linewidth,keepaspectratio]{figures/batchgemm.pdf}
    \caption{Splitting and merging matrix multiplications.}
    \vspace{-1em}
    \label{fig:batchgemm}
\end{figure}

A typical example of expression splitting and merging are the transformation between {\tt Matmul} and {\tt BatchMatmul}: multiple matrix multiplications can be merged together to a single batch matrix multiplication, which can be splitted into multiple matrix multiplications, as shown in \Cref{fig:batchgemm}.

\para{Expression fusion} fuses multiple dependent expressions into one using the following rule:
\begin{align*}
\opL_{\vec{y}}^{\mathbb{Y}}g(\tensors{T'}\posB{\vec{y}}) \circ
\opL_{\vec{x}}^{\mathbb{X}}f(\mathT\pos{\vec{x}}) \Longrightarrow
\opL_{\vec{y}}^{\mathbb{Y}}g(\{\opL_{\vec{x}}^{\mathbb{X}}f(\mathT\pos{\vec{x}})\}\posB{\vec{y}})
\end{align*}
where $\circ$ denotes that the result of latter expression will be fed as the input of the former expression, i.e., $\tensors{T'}$ equals to the computation result of $\opL_{\vec{x}}^{\mathbb{X}}f(\mathT\pos{\vec{x}})$.

Expression fusion allows \sys{} to consider {\em operator fusion}, a commonly used technique that optimizes tensor programs by fusing the computation of multiple operators into a single kernel to reduce data movement and kernel launch overhead.
For example, a {\tt Conv} operator followed by a {\tt ReLU} operator can be fused into a {\tt Conv+ReLU} operator.


==> rules2.tex <==
\section{Tensor Algebra Expression}
\label{sec:expression}
\sys represents a tensor program as a {\em tensor algebra expression} that defines how to compute each element of the output tensor from input tensors.
For example, \Cref{fig:expr} shows the expression for multiplying three matrices. We now explain the components of an expression.



\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/expr.pdf}
    \vspace{-2em}
    \caption{Example tensor algebra expressions for two matrix multiplications $A\times B\times C$. The red box highlights a \stage that instantiates the intermediate result of $A\times B$.}
    \label{fig:expr}
    \vspace{-1.5em}
\end{figure}

\para{Traversal and summation notations.} A {\em traversal notation}, denoted as $\opLd_{x=x_0}^{x_1}$, consists of an {\em iterator} $x$ and an {\em iterating space} $[x_0, x_1)$.
The traversal notation corresponds to a dimension of the output tensor, where the iterating space is the range of the dimension. 
The order between different traversal notations indicates the layout of the output tensor.
E.g., in \Cref{fig:expr}, $\opLd_{c=0}^{C}$ followed by $\opLd_{r=0}^{R}$ shows that the expression's output is a 2-dimensional tensor with a shape $C\times R$.

A {\em summation notation}, denoted as
$\sumd_{x=x_0}^{x_1}$, corresponds to a dimension with range $[x_0, x_1)$ that is iterated over when computing each output element. In \Cref{fig:expr}, the summation notation $\sumd_{k_0=0}^{K}$ indicates that the computation for each output element iterates over an interval with $K$ elements.
Note that \sys's expression notation is invariant under permutation of summation notations, which corresponds to different {\em schedules} of an expression and therefore is not considered in the expression search space.

Tensors are indexed by a {\em linear combination} of multiple iterators 
or the division or remainder of iterators (e.g., $h\%2$).
For simplicity, we may merge multiple iterators into one iterator vector in the paper. 
Iterator space also can be denoted by an integer set or omitted in expressions. 
For example, $\opLd_{c=0}^{C}\opLd_{r=0}^{R}$ can be represented as $\opLd_{cr}$ or $\opLd^{\mathbb{X}}_{\vec{x}}$, where $\vec{x}=(c,r)$ and $\mathbb{X}=\mathbb{C}\times\mathbb{R}$ is the iterating space. 

\para{Scope.} For a tensor program with multiple operators (e.g., two consecutive matrix multiplications $A\times B \times C$), a common optimization is to instantiate and reuse intermediate results (e.g., caching the output of $A\times B$), which avoids repetitive computation for these results. \sys introduces \stages to represent the instantiation of intermediate results and enable their reuse. Formally, a tensor algebra expression is a {\em \stage}, denoted by a surrounding $\big\{\big\}$, if the output of the expression is instantiated into a tensor, which allows subsequent computation to refer to its output as a tensor and therefore avoids repeated computation of its output.
In \Cref{fig:expr}(b), the expression corresponding to $A\times B$ becomes a \stage, which allows subsequent computation to directly refer to the output of this expression as a tensor.

Most of \sys's derivation rules (described in \Cref{sec:rules}) are based on transformations between \stages, including generating new \stages from existing ones, transforming a \stage to another form, and merging multiple \stages into one.
Transformations between scopes are essential to \sys's performance optimizations. 

\para{Padding}
Tensors may have paddings.
For example, convolution may access input tensors at a position outside of $A$'s region.
We call these positions the paddings of $A$, whose elements are $0$ if not specified.

\para{General format.}
We represent arbitrary 1-\stage expressions in the following format:
\vspace{\alignvspacetop}
\begin{align*}
    \opL_{\vec{x}}^{\mathbb{X}}\sum_{\vec{y}}^{\mathbb{Y}}f(\mathT\pos{\vec{x},\vec{y}})
    \\[\alignvspacebottom]
\end{align*}
where $\mathT=\{T_0, T_1, ...\}$ is a list of input tensors, $\tau(\vec{x},\vec{y})$ is the indexing function that computes an element index for $\mathT$ using iterators $\vec{x}$ and $\vec{y}$, and $f$ is the computation taking on the indexed elements of $\mathT$.

\section{Derivation Rules}
\label{sec:rules}

\begin{table*}[h]
\centering
\caption{Derivation rules for tensor algebra expressions}
\label{tab:derivation-rules}
\vspace{-0.5em}
\small
\begin{tabular}{cll}
\toprule
& Rules & Descriptions \\ \midrule

\multirow{3}{*}{\shortstack[m]{Inter-expression \\ derivation}}  & Expression splitting & Split an expression into multiple independent expressions \\ 
& Expression merging & Merge multiple independent expressions into one \\ 
& Expression fusion & Fusing multiple dependent expressions into one \\ 
\midrule

\multirow{5}{*}{\shortstack[m]{Intra-expression \\ derivation}} 
& Summation splitting & Split summation from one \stages into two  \\ %
& Variable substitution & Replace iterators of traversal notations with new ones \\ %
& Traversal merging & Merge two \stages into one by merging traversals  \\ %
& Boundary relaxing & Relax the range of iterators \\ 
& Boundary tightening  & Tighten  the range of iterators \\ 
\midrule

\multirow{2}{*}{\shortstack[m]{Expression \\ instantiation}} 
& Operator matching & Match a \stage with operators and replace it by a tensor \\
& \eop generation & Generate an \eop for a scope and replace it by a tensor \\ 
\bottomrule
\end{tabular}%
\vspace{-1em}
\end{table*}


To discover highly-optimized expressions for an input tensor program, \sys uses {\em derivation rules} to apply transformations on an input expression.
\Cref{tab:derivation-rules} summarizes the derivation rules used by \sys, which are divided into three categories.
The proof of these rules are provided in Appendix.

\subsection{Inter-Expression Derivation}
\label{sec:inter-expr-rule}

\para{Expression splitting} divides an expression into two independent expressions by partitioning the traversal space of the expression $\mathbb{X}$ into two subspaces $\mathbb{X}_1$ and $\mathbb{X}_2$ such that $\mathbb{X} \subseteq \mathbb{X}_1 \cup \mathbb{X}_2$. The expression splitting rule is as follows: 
\vspace{\alignvspacetop}
\begin{align*}
\opL_{\vec{x}}^{\mathbb{X}}f(\mathT\pos{\vec{x}}) \Longrightarrow 
\opL_{\vec{x}}^{\mathbb{X}_1}f(\mathT\pos{\vec{x}}) \sim \opL_{\vec{x}}^{\mathbb{X}_2}f(\mathT\pos{\vec{x}}) 
\\[\alignvspacebottom]
\end{align*}
where $\sim$ denotes the independence of the two expressions. 

\para{Expression merging} combines two independent expressions that have identical computation into a single expression by merging the traversal spaces of the original expressions:
\vspace{\alignvspacetop}
\begin{align*}
\opL_{\vec{x}}^{\mathbb{X}_1}f(\mathT\pos{\vec{x}}) \sim \opL_{\vec{x}}^{\mathbb{X}_2}f(\mathT\pos{\vec{x}}) \Longrightarrow \opL_{\vec{x}}^{\mathbb{X}}f(\mathT\pos{\vec{x}})
\\[\alignvspacebottom]
\end{align*}
where $\mathbb{X}_1 \cup \mathbb{X}_2 \subseteq \mathbb{X}$. Expression merging is the symmetric transformation of expression splitting.

\begin{figure}[]
    \centering
    \includegraphics[width=\linewidth,keepaspectratio]{figures/batchgemm.pdf}
    \vspace{-2em}
    \caption{Splitting and merging matrix multiplications.}
    \label{fig:batchgemm}
    \vspace{-2em}
\end{figure}

A typical example of expression splitting and merging is the transformation between {\tt Matmul} and {\tt BatchMatmul}: multiple matrix multiplications can be merged together to a single batch matrix multiplication, and a batch matrix multiplication can be split into multiple matrix multiplications, as shown in \Cref{fig:batchgemm}.

\para{Expression fusion} fuses multiple dependent expressions into one using the chain rule:
\aligntop
\begin{align*}
\opL_{\vec{y}}^{\mathbb{Y}}g(\tensors{T'}\posB{\vec{y}}) \circ
\opL_{\vec{x}}^{\mathbb{X}}f(\mathT\pos{\vec{x}}) \Longrightarrow
\opL_{\vec{y}}^{\mathbb{Y}}g(\{\opL_{\vec{x}}^{\mathbb{X}}f(\mathT\pos{\vec{x}})\}\posB{\vec{y}})
\alignbottom
\end{align*}
where $\m{E}_1\circ\m{E}_2$ denotes that the result of  expression $\m{E}_2$ is fed as inputs to expression $\m{E}_1$ (i.e., $\tensors{T'}$ equals to the computation result of $\opL_{\vec{x}}^{\mathbb{X}}f(\mathT\pos{\vec{x}})$).

Expression fusion allows \sys{} to consider {\em operator fusion}, a technique that fuses the computation of multiple operators into a single kernel to reduce data movement and kernel launch overhead.


\begin{figure*}[h!]
    \centering
    \includegraphics[width=0.95\linewidth,keepaspectratio]{figures/conv2gemm-expr.pdf}
    \vspace{-1em}
    \caption{The derivation process of the example in \Cref{fig:conv2gemm}, which replaces {\tt Conv} with {\tt Matmul} and \eops}
    \label{fig:conv2gemm-expr}
    \vspace{-1.5em}
\end{figure*}

\subsection{Intra-Expression Derivation}
\label{sec:compute-rule}
Intra-expression derivation rules transform an expression into other functionally equivalent forms, which is essential for constructing a comprehensive search space of expressions for a tensor program.
 \Cref{fig:conv2gemm-expr} shows the intra-expression derivation rules used to discover the optimization in \Cref{fig:conv2gemm}. We now describe these intra-expression derivation rules.


\para{Summation splitting} divides a summation $\sum_{\vec{s}}$ in an expression into two summations $\sum_{\vec{s_1}}$ and $\sum_{\vec{s_2}}$ and instantiates the result of the inner summation by converting it to a \stage:
\vspace{-0.5em}
\begin{align*}
 \opL_{\vec{x}}\sum_{\vec{s_1},\vec{s_2}}f(\mathT\pos{\vec{x},\vec{s_1},\vec{s_2}})\Rightarrow\opL_{\vec{x}}\sum_{\vec{s_1}}\big\{\opL_{\vec{x}\vec{s_1}}\sum_{\vec{s_2}}f(\mathT\pos{\vec{x},\vec{s_1},\vec{s_2}})\big\}[\vec{x},\vec{s_1}]
\end{align*}\\[-1.3em]
where $\mathbf{\tau}$ is a mapping from $(\vec{x}, \vec{s_1}, \vec{s_2})$ to an input position.
\sys divides the iterators of a summation into two disjoint groups, $\vec{s_1}$ and $\vec{s_2}$, which splits the summation into two nested \stages $\m{S}_1, \m{S}_2$, where $\m{S}_1=\opLd_{\vec{x}\vec{s_1}}\sumd_{\vec{s_2}}f(\mathT\pos{\vec{x},\vec{s_1},\vec{s_2}})$ and $\m{S}_2=\opLd_{\vec{x}}\sumd_{\vec{s_1}}\m{S}_1[\vec{x},\vec{s_1}]$.
Note that in summation splitting, \sys converts the result of the inner summation into a \stage, whose output is reused by the outer summation.

To transform a 3$\times$3 convolution to a batch of nine matrix multiplications, as shown in \Cref{fig:conv2gemm-expr}, \sys first transforms the initial expression $\m{E}_1$ to $\m{E}_2$ by splitting the summation $\sum_{crs}$ into two operations $\sum_{rs}$ and $\sum_{c}$, and instantiating the output of the inner summation 
(i.e., \big\{$\opL_{rshwf}\sum_{c}A[h+r,w+s,c]K[r,s,f,c]$\big\}).
The inner \stage only sums along the $c$ dimension; as a result, an intermediate $5$-dimensional tensor is instantiated since the summation along the $r$ and $s$ dimensions is not performed but converted to traversal notations.
The outer \stage computes the remaining summation over the $r$ and $s$ dimensions, which produces a $4$-dimensional tensor.
\Cref{fig:conv2gemm-expr} (a) and (b) depict the computation graphs before and after this derivation.





\para{Variable substitution} substitutes a set of traversal iterators $\opL_{\vec{x}}$ with a new set of iterators $\opL_{\vec{y}}$ by applying a {\em bijective} function $\Phi$ (i.e., $\vec{y}=\Phi(\vec{x})$).\footnote{A mapping function $\Phi$ is {\em bijective} if it is both injective (one-to-one) and surjective (onto).}
This transformation allows the expression to be computed using a different set of traversal iterators. In particular, for an expression $\opL_{\vec{x}}^{\mathbb{X}}f(\mathT[\tau(\vec{x})])$, variable substitution introduces an intermediate \stage that computes $\opL_{\vec{y}}^{\mathbb{Y}}f(\mathT[\tau(\Phi^{-1}(\vec{y}))])$, where $\Phi$ is a bijective function that maps $\mathbb{X}$ to $\mathbb{Y}=\Phi(\mathbb{X})$, and $\Phi^{-1}$ is the reverse function of $\Phi$. Formally,
\aligntop
\begin{align*}
\opL_{\vec{x}}^\mathbb{X}f(\mathT\pos{\vec{x}})\Rightarrow\opL_{\vec{x}}^\mathbb{X}\{\opL_{\vec{y}}^{\Phi(\mathbb{X})}f(\mathT\pos{\Phi^{-1}(\vec{y})})\}[\Phi(\vec{x})]
\alignbottom
\end{align*}
Variable substitution constructs an intermediate \stage with new traversal iterators.
To preserve functional equivalence, the original iterator $\vec{x}$ is used to construct the final result using the output of the intermediate \stage.


In \Cref{fig:conv2gemm-expr}, \sys applies variable substitution to transform the expression from $\m{E}_2$ to $\m{E}_3$, using bijective function: $\Phi(r,s,h,w,f)=(r,s,f,h+r,w+s)$. 
Specifically, $h+r$ and $w+s$ are substituted with $t_1$ and $t_2$ in $\m{E}_3$.
Note that variable substitution does not change the computation graph.



\para{Traversal merging} merges the traversal notations in two \stages into a single \stage using a bijective function $\Phi$:
\aligntop
\begin{align*}
\opL_{\vec{x}}^\mathbb{X}\sum_{\vec{y}}^\mathbb{Y}\{\opL_{\vec{z}}^\mathbb{Z}f(\mathT\pos{\vec{z})}\}[\Phi(\vec{x},\vec{y})]\Rightarrow\opL_{\vec{x}}^\mathbb{X}\sum_{\vec{y}}^\mathbb{Y}f(\mathT\pos{\Phi(\vec{x},\vec{y})})
\alignbottom
\end{align*}
where $\Phi(\mathbb{X}\times \mathbb{Y}) \subseteq \mathbb{Z}$. 

For the example in \Cref{fig:conv2gemm-expr}, \sys applies traversal merging to transform $\m{E}_4$ to $\m{E}_5$.
For this transformation, the outer traversal and summation notations and the inner traversal notation both include five iterators (i.e., $\vec{x}=(h,w,f)$, $\vec{y}=(r,w)$, and $\vec{z}=(r,s,h,w,f)$).
Traversal merging is applied with an identity mapping function $\Phi$ and an indexing function $\tau(r,s,h,w,f)=(r,s,f,h+r,w+s)$.
Traversal merging removes a \stage while preserving the computation graph.








\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth,keepaspectratio]{figures/conv5x5-graph.pdf}
    \vspace{-2em}
    \caption{\texttt{Conv5x5} to \texttt{Conv3x3} in SRCNN \lz{Explained in the rule}}
    \vspace{-2em}
    \label{fig:conv5x5}
\end{figure}

\para{Boundary relaxing and tightening} inspect whether the computation for some output elements can be avoided if these elements are constants for arbitrary inputs.
\sys executes constant propagation on expressions to deal with constant numbers in expressions and padding in tensors.
If a region of output has constant value, \sys converts it into an attribute of tensors to reduce meaningless computation. 
The following formula shows how boundary relaxing and tightening are performed:
\vspace{-1.2em}
\begin{align*}
\opL_{\vec{x}}^\mathbb{X}f(\mathT\pos{\vec{x}}) \Longleftrightarrow \opL_{\vec{x}}^{\mathbb{X}'}f(\mathT\pos{\vec{x}})
\alignbottom
\end{align*}
, where $\mathbb{X} \subset \mathbb{X}'$, and computation on $\mathbb{X}' - \mathbb{X}$ will not be used as the results of the tensor program. 

In the running example in \Cref{fig:conv2gemm-expr}, the formula in $\m{E}_4$ performs boundary relaxing on $t_1$ and $t_2$, transforming their ranges from $[0, H+r)$ and $[0, W+s)$ to $[-1, H+1)$ and $[-1, W+1)$, respectively, as $r$ and $s$ are in range of $[-1, 1]$. 
After boundary relaxing, the computation graph is transformed from \Cref{fig:conv2gemm-expr} (b) to (c).
The formula in $\m{E}_6$ performs boundary tightening on on $t_1$ and $t_2$, transforming their ranges from $[-1, H+1)$ and $[-1, W+1)$ to $[0, H)$ and $[0, W)$, respectively, as the computation taken on $t_1 = -1$, $t_1 = H+1$, $t_2 = -1$ and $t_2 = W+1$ will not be used for the output tensor.
After boundary tightening, the computation graph is transformed from \Cref{fig:conv2gemm-expr} (c) to (d).





































\subsection{Expression Instantiation}
\label{sec:expre-contraction}

Expression instantiation rules lower expressions into executable kernels.
After applying these rules, the instantiated scope is replaced with a tensor in the original expression and separated from the following derivation. 
\sys supports two classes of instantiation, operator matching and \eop generation, to leverage existing highly optimized kernels and flexibly generate other kernels.  
In this subsection, we will introduce how these two instantiation rules work.


\begin{table}[]
\caption{\Itab}
\label{tab:itab}
\vspace{-0.5em}
\centering
\small
\begin{tabular}{ccc|cccc}
\toprule
\multicolumn{3}{c|}{Tensors}          & \multicolumn{4}{c}{Ops} \\
\hline
input      & weight     & output     & \texttt{Add} & \texttt{Matmul}  & \texttt{Conv}  & \texttt{G2BMM} \\
\hline
\checkmark & \checkmark & \checkmark & $mn$  & $b$       &       & $bm$    \\
\checkmark &            & \checkmark &     & $m$       & $nhw$   &       \\
           & \checkmark & \checkmark &     & $n$       & $f$     & $w$     \\
\checkmark & \checkmark &            &     & $k$       & $crs$   & $k$     \\
\bottomrule
\end{tabular}
\vspace{-2em}
\end{table}

\subsubsection{new Pattern Matching}
\label{sec:rule-pattern-matching}

Mapping a tensor algebra expression to an operator is challenging since an operator can be represented in various expressions with potentially different tensor layouts, tensor dimensions, and iterators.
For example, the standard tensor algebra expression of a batched matrix multiplication is shown in Expression~(\ref{eq:bmm}). 
However, although Expression~(\ref{eq:bmm-variant}) is significantly different from Expression~(\ref{eq:bmm}), it can also be directly instantiated as a batched matrix multiplication in math libraries\footnote{Math libraries including BLAS allow for different input layouts by specifying the stride of tensor dimensions.}. Similar problems exist for other operators. 

\aligntop
\begin{align}
    &\opL_{bmn}\sum_{k}A[b,m,k]B[b,k,n]
    \label{eq:bmm} \\
    &\opL_{uvw}\sum_{x}C[u,0,v,x+1]D[u-1,u,x,w]
    \label{eq:bmm-variant}
\end{align}\alignbottom



To match a tensor algebra expression to operators, 
\sys uses {\em \itab} to summarize linear algebra properties of expressions.
\Itab supports all operators expressible in tensor algebra expression. \Cref{tab:itab} shows typical operators, including an element-wise operator, matrix multiplication, convolution, and G2BMM~\cite{langer2018band} (general to band matrix multiplication). 
The right part of the table list all iterators of an operator, which are categorized into four groups based on whether the iterators appears in the indexes of input, weight, and output tensors. 
\Itab also records the coefficient of iterators in the index of each tensors for operator matching.

\aligntop
\begin{align}
    B[b,k,n] &\Rightarrow B[l_{B0}b+l_{B1}k+n]\\
    D[u-1,u,x,w] &\Rightarrow D[(l_{D0}+l_{D1})u+l_{D2}x+w-l_{D0}]
    \label{eq:bmm-index}
\end{align}\alignbottom

Taking the batched matrix multiplication in Expression~(\ref{eq:bmm}) as an example, the iterators $b$, $m$, $n$, and $k$ appear in different combinations of the input, weight, and output tensors.
These variables are assigned to different \emph{iterator groups}, as shown in \Cref{tab:itab}.
To match an expression with a specific operator, we need to match the iterators in this expression to the iterators in the \itab.

The detailed matching process is listed as follows:

\begin{enumerate}[leftmargin=*]
    \item  \textbf{Fill iterators into \itab}: enumerate all the iterators in a given expression, and fill them in into the iterator groups in the \itab according to which tensor it appears in. 
    
    \item \textbf{Match iterator groups}: for each iterator group in \itab, the number of iterators should be the same.
    
    \item \textbf{Match iterators}: if there are multiple iterators in an iterator group, enumerate all one-to-one mapping between variables of the operator and those of the expression. 
    After the variables are mapped, check whether the coefficients of iterators in index match (whether the coefficient of each variable and the correlation between different variables in the expression are consistent with patterns, e.g., $h$ and $r$ should have the same coefficient in the index of input tensor of convolution in Expression~$\m{E}_1$ in \Cref{fig:conv2gemm-expr}). 
    
\end{enumerate}

For the example in Equation~(\ref{eq:bmm-variant}), it has the same iterator groups with \texttt{Matmul}. There is an unique one-to-one iterator mapping between the expression and \texttt{Matmul} and it matches all iterators.
After the pattern match rule succeeds, \sys replaces the matched scope with a tensor and generates a corresponding \texttt{Matmul} operator in the computation graph.

\subsubsection{Pattern Matching}
\label{sec:rule-pattern-matching}

Mapping a tensor algebra expression to an operator is challenging since an operator can be represented in various expressions with potentially different tensor layouts, tensor dimensions, and iterators.
For example, the standard tensor algebra expression of a batched matrix multiplication is shown in Expression~(\ref{eq:bmm}). 
However, although Expression~(\ref{eq:bmm-variant}) is significantly different from Expression~(\ref{eq:bmm}), it can also be directly instantiated as a batched matrix multiplication in math libraries\footnote{Math libraries including BLAS allow for different input layouts by specifying the stride of tensor dimensions.}. Similar problems exist for other operators. 
\aligntop
\begin{align}
    \opL_{bmn}\sum_{k}A[b,m,k]B[b,k,n]
    \label{eq:bmm}
\end{align}\\[-2.8em]
\begin{align}
    \opL_{bmn}\sum_{k}C[b,0,m,1+k]D[b-1,b,k,n]
    \label{eq:bmm-variant}
\end{align}\alignbottom



To match a tensor algebra expression to operators, 
\sys uses {\em \itab} to summarize linear algebra properties of expressions.
\Itab supports all operators expressible in tensor algebra expression. \Cref{tab:itab} shows typical operators, including an element-wise operator, matrix multiplication, convolution, and G2BMM~\cite{langer2018band} (general to band matrix multiplication). 
The right part of the table list all iterators of an operator, which are categorized into four groups based on whether the iterators appears in the indexes of input, weight, and output tensors. 
\Itab also records the coefficient of iterators in the index of each tensors for operator matching.

Taking the batched matrix multiplication in Expression~(\ref{eq:bmm}) as an example, the iterators $b$, $m$, $n$, and $k$ appear in different combinations of the input, weight, and output tensors.
These variables are assigned to different \emph{iterator groups}, as shown in \Cref{tab:itab}.
To match an expression with a specific operator, we need to match the iterators in this expression to the iterators in the \itab.

The detailed matching process is listed as follows:

\begin{enumerate}[leftmargin=*]
    \item  \textbf{Fill iterators into \itab}: enumerate all the iterators in a given expression, and fill them in into the iterator groups in the \itab according to which tensor it appears in. 
    
    \item \textbf{Match iterator groups}: for each iterator group in \itab, the number of iterators should be the same.
    
    \item \textbf{Match iterators}: if there are multiple iterators in an iterator group, enumerate all one-to-one mapping between variables of the operator and those of the expression. 
    After the variables are mapped, check whether the coefficients of iterators in index match (whether the coefficient of each variable and the correlation between different variables in the expression are consistent with patterns, e.g., $h$ and $r$ should have the same coefficient in the index of input tensor of convolution in Expression~$\m{E}_1$ in \Cref{fig:conv2gemm-expr}). 
    
\end{enumerate}

For the example in Equation~(\ref{eq:bmm-variant}), it has the same iterator groups with \texttt{Matmul}. There is an unique one-to-one iterator mapping between the expression and \texttt{Matmul} and it matches all iterators.
After the pattern match rule succeeds, \sys replaces the matched scope with a tensor and generates a corresponding \texttt{Matmul} operator in the computation graph.

\subsubsection{\eop Generation}
\label{sec:rule-eop-matching}

For expressions which cannot match existing operators, \sys converts them into \eops and generates executable kernels based on their tensor algebra expressions.
Since tensor algebra expressions exactly define the computation semantics, 
\sys is able to feed them into existing code generation frameworks, such as TVM, Halide, and Tiramisu~\cite{baghdadi2019tiramisu}.
For example, for the expression in $\m{E}_7$  of \Cref{fig:conv2gemm-expr}, \sys lowers it to TVM by converting its iterator space of traversal notation into a tensor and the computation expression into a lambda function.
\Cref{fig:codegen} shows the result which can be processed by TVM to automatically generate kernel.

\begin{figure}[h]
    \centering
    \vspace{-0.5em}
    \includegraphics[width=\linewidth,keepaspectratio]{figures/codegen-tvm.pdf}
    \vspace{-2em}
    \caption{Lowering $\m{E}_7$ in \Cref{fig:conv2gemm-expr} to TVM.}
    \label{fig:codegen}
    \vspace{-2em}
\end{figure}

\subsubsection{Discussion}

Although \sys can treat arbitrary expressions as \eops to support various optimizations, the code generation process introduces too much overhead making such optimizations impractical.
Considering existing DNN libraries already provide many predefined operators which can outperform generated kernels in most cases, \sys adopts the strategy that mapping the expression to the combination of compute-bound predefined operators and memory-bound \eops.
In this way, \sys can benefit from both the efficiency of existing libraries and the flexibility of auto-generated \eops.
Moreover, tuning memory-bound operators is much easier than tuning compute-bound ones since the former ones often have much easier schedules. 
This guarantees \sys can find optimized transformations within a promising time.
Typically, \sys spends around one minute to generate a memory-bound \eops.

